Multitask Learning for Time Series Data with 2D Convolution

Multitask learning (MTL) aims to develop a unified model that can handle a set of closely related tasks simultaneously. By optimizing the model across multiple tasks, MTL generally surpasses its non-MTL counterparts in terms of generalizability. Although MTL has been extensively researched in various domains such as computer vision, natural language processing, and recommendation systems, its application to time series data has received limited attention. In this paper, we investigate the application of MTL to the time series classification (TSC) problem. However, when we integrate the state-of-the-art 1D convolution-based TSC model with MTL, the performance of the TSC model actually deteriorates. By comparing the 1D convolution-based models with the Dynamic Time Warping (DTW) distance function, it appears that the underwhelming results stem from the limited expressive power of the 1D convolutional layers. To overcome this challenge, we propose a novel design for a 2D convolution-based model that enhances the model's expressiveness. Leveraging this advantage, our proposed method outperforms competing approaches on both the UCR Archive and an industrial transaction TSC dataset.

==> insert/fig_hard_soft.tex <==
\begin{figure}[ht]
\centerline{
\includegraphics[width=0.99\linewidth]{insert/figure/fig_hard_soft_0.pdf}
}
\caption{
% \footnotesize
Hard parameter sharing has more shared layers compared to soft parameter sharing; therefore, the total number of layers will be less in hard parameter sharing compared to soft parameter sharing.
}
\label{fig:hard_soft_share}
\end{figure}


==> insert/fig_resnet_2d_use.tex <==
\begin{figure}[ht]
\centerline{
\includegraphics[width=0.99\linewidth]{insert/figure/fig_resnet_2d_use_0.pdf}
}
\caption{
% \footnotesize
The figure shows how the proposed \texttt{ResNet2D} model is used for both distance learning and MTL experiments.
}
\label{fig:resnet_2d_use}
\end{figure}


==> insert/tab_ucr_data.tex <==
\begin{table*}[t]
\centering
\caption{
The performances of different methods are compared at dataset level.
The number in the table are the average rank across all tasks within a dataset (i.e., the smaller the better).
The proposed method is the best or the second best in 5 out of 7 datasets.
}
\label{tab:ucr_data}
% \resizebox{0.99\columnwidth}{!}{
\footnotesize
\begin{tabular}{l||c|cc|cc}
Dataset & 1NN-DTW & ResNet1D & ResNet2D & \begin{tabular}[c]{@{}l@{}}ResNet1D \\      w/ MTL\end{tabular} & \begin{tabular}[c]{@{}l@{}}ResNet2D \\      w/ MTL\end{tabular} \\ \hline \hline
Cricket & \underline{2.17} & 2.83 & 3.50 & 4.83 & \textbf{1.67} \\
UWaveGestureLibrary & 4.50 & 2.88 & \underline{1.75} & 4.25 & \textbf{1.63} \\
AllGestureWiimote & \textbf{1.33} & \underline{1.67} & 4.00 & 4.67 & 3.33 \\
DodgerLoop & \textbf{2.00} & 4.00 & \textbf{2.00} & 3.83 & 3.17 \\
SemgHand & 3.83 & 4.83 & \underline{2.33} & 3.00 & \textbf{1.00} \\
GestureMidAir & \underline{2.17} & 4.67 & 3.00 & 3.50 & \textbf{1.67} \\
ECG & 4.58 & \textbf{1.83} & 2.67 & 3.33 & \underline{2.58} \\
\end{tabular}
\end{table*}
